Spatio-Temporal Few-Shot Learning via Diffusive Neural Network Generation

Spatio-temporal modeling is foundational for smart city applications, yet it is often hindered by data scarcity in many cities and regions. To bridge this gap, we propose a novel generative pre-training framework, GPD, for spatio-temporal few-shot learning with urban knowledge transfer. Unlike conventional approaches that heavily rely on common feature extraction or intricate few-shot learning designs, our solution takes a novel approach by performing generative pre-training on a collection of neural network parameters optimized with data from source cities. We recast spatio-temporal few-shot learning as pre-training a generative diffusion model, which generates tailored neural networks guided by prompts, allowing for adaptability to diverse data distributions and city-specific characteristics. GPD employs a Transformer-based denoising diffusion model, which is model-agnostic to integrate with powerful spatio-temporal neural networks. By addressing challenges arising from data gaps and the complexity of generalizing knowledge across cities, our framework consistently outperforms state-of-the-art baselines on multiple real-world datasets for tasks such as traffic speed prediction and crowd flow prediction. The implementation of our approach is available: https://github.com/tsinghua-fib-lab/GPD.

==> tables/compare.tex <==
\begin{table}[t]
% \small
% \setlength\tabcolsep{2pt}
\centering
\begin{tabular}{ccccccc}
\hline
\textbf{Models} &
  \textbf{\# Source cities} &
 \textbf{ Matching} &
  
  \textbf{Joint train} &
 \textbf{ Few-shot} &
  \textbf{Zero-shot} &
  \textbf{xxx} \\ \hline
RegionTrans & \ding{55} & \ding{55}  & \ding{55}  & \checkmark & \ding{55}  & \ding{55} \\ \hline
MetaST & \ding{55} & \ding{55}  & \ding{55}  & \checkmark & \ding{55}  & \ding{55} \\ \hline
CrossTReS & \ding{55} & \ding{55}  & \ding{55}  & \checkmark & \ding{55}  & \ding{55} \\ \hline
DASRNet & \ding{55} & \ding{55}  & \ding{55}  & \checkmark & \ding{55}  & \ding{55} \\ \hline
ST-GFSL & \ding{55} & \ding{55}  & \ding{55}  & \checkmark & \ding{55}  & \ding{55} \\ \hline
TransGTR & \ding{55} & \ding{55}  & \ding{55}  & \checkmark & \ding{55}  & \ding{55} \\ \hline
\end{tabular}
\caption{Comparison of approaches for urban transfer learning.}
\label{tbl:compare}
\end{table}


==> tables/crowd_zero_shot.tex <==
\begin{table}[t]
\renewcommand{\arraystretch}{1.2}
\centering
\begin{tabular}{ccccccccc}
\toprule
 & \multicolumn{2}{c}{\textbf{DC}} & \multicolumn{2}{c}{\textbf{BM}} & \multicolumn{2}{c}{\textbf{man}} 
 \\ \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} 
\textbf{Model} & \textbf{MAE}      & \textbf{RMSE}     & \textbf{MAE}      & \textbf{RMSE}     & \textbf{MAE}      & \textbf{RMSE}       \\ 
\cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
TPB & 139.754  & 145.019 & 83.24 & 84.731 & 217.86 &  224.045   \\ 
DASTNet  & 32.075  & 57.807 & 83.24 & 84.731 & 56.433 & 73.239    \\ 
MAML & 31.485 & 65.885 & 16.663 & 30.402 & 67.86 &    99.143  \\ 
STGFSL  & 44.431 & 65.236 & 19.699 & 35.728 & 48.35 & 74.904   \\ 
\cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}  
Ours    & 26.771 & 50.960  & 16.357 & 24.494 & 42.476 & 60.830  \\ 


\bottomrule
\end{tabular}
\caption{Performance comparison of zero-shot scenarios on four crowd flow datasets in terms of MAE and RMSE. Bold denotes the best results and \underline{underline} denotes the second-best results.}
\label{tbl:main_zero_crowd}
\end{table}

==> tables/model_cmp_step.tex <==
\begin{table}[t]
\centering
\begin{tabular}{ccccccc}
\toprule

& \multicolumn{3}{c}{\textbf{MAE}} & \multicolumn{3}{c}{\textbf{RMSE}}
\\ 
 \cmidrule(lr){2-4} \cmidrule(lr){5-7} 
\textbf{STG Model} & \textbf{Step 1}     & \textbf{Step 3} & \textbf{Step 6}
& \textbf{Step 1}    & \textbf{Step 3} & \textbf{Step 6}
\\ 
\cmidrule(lr){1-1} \cmidrule(lr){2-4} \cmidrule(lr){5-7} 

STGCN     & & & & & &  \\
GWN      & & & & & & \\ 
 \bottomrule
\end{tabular}
\caption{Performance comparison of different STG models on Washington D.C. dataset at different prediction steps in terms of MAE and RMSE.}
\label{tbl:sup_model_cmp_step}
\end{table}

==> tables/traffic_few_shot.tex <==
\begin{table}[t]
\renewcommand{\arraystretch}{1.2}
\centering
\begin{tabular}{ccccc}
\toprule
 & \multicolumn{2}{c}{\textbf{METR-LA}} & \multicolumn{2}{c}{\textbf{Didi-Chengdu}} 
 \\ \cmidrule(lr){2-3} \cmidrule(lr){4-5} 
\textbf{Model} & \textbf{MAE}      & \textbf{RMSE}     & \textbf{MAE}      & \textbf{RMSE}      \\ 
\cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-5}
HA    &      &      &    &        \\
ARIMA    &      &      &    &    \\
RegionTrans  &   &      &      &     \\
TPB     &     &      &      &    \\
DASTNet     &     &      &      &       \\ 
MAML     &    &      &      &    \\ 
STGFSL     &     &      &      &   \\ 
\cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-5}
GPD     &    &      &      &     \\ 
\bottomrule
\end{tabular}
\caption{Performace comparison of few-shot scenarios on four traffic speed datasets in terms of MAE and RMSE. Bold denotes the best results and \underline{underline} denotes the second-best results.}
\label{tbl:main_few_traffic}
\end{table}

==> tables/traffic_zero_shot.tex <==
\begin{table}[t]
\renewcommand{\arraystretch}{1.2}
\centering
\begin{tabular}{ccccccccc}
\toprule
 & \multicolumn{2}{c}{\textbf{PEMS-BAY}} & \multicolumn{2}{c}{\textbf{METR-LA}} & \multicolumn{2}{c}{\textbf{Didi-Chengdu}}  & \multicolumn{2}{c}{\textbf{Didi-Shenzhen}}  
 \\ \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}  \cmidrule(lr){8-9} 
\textbf{Model} & \textbf{MAE}      & \textbf{RMSE}     & \textbf{MAE}      & \textbf{RMSE}     & \textbf{MAE}      & \textbf{RMSE}    & \textbf{MAE}      & \textbf{RMSE}      \\ 
\cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
TPB     & 17.409 & 18.441 & 31.577 & 33.976  & 26.715 & 31.393 & 7.249 & 10.158    \\
DASTNet     &     &      &      &    &     &        & &        \\ 
MAML     & 62.513 & 63.228 & 57.966 & 59.527 & 28.969 & 30.505 & 29.978 & 31.950  \\ 
STGFSL     & 32.489 & 33.209 & 39.010 & 40.425 & 7.760 & 10.280 & 14.530 & 17.702 \\ 
\cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
GPD     & 5.595 & 9.364 & 8.899 & 12.783 & 7.76 & 10.28 & 6.226 & 8.031  \\ 
\bottomrule
\end{tabular}
\caption{Performace comparison of zero-shot scenarios on four traffic speed datasets in terms of MAE and RMSE. Bold denotes the best results and \underline{underline} denotes the second-best results.}
\label{tbl:main_zero_traffic}
\end{table}
